EARL: Eye-on-Hand Reinforcement Learner for Dynamic Grasping with Active Pose Estimation

In this paper, we explore the dynamic grasping of moving objects through active pose tracking and reinforcement learning for hand-eye coordination systems. Most existing vision-based robotic grasping methods implicitly assume target objects are stationary or moving predictably. Performing grasping of unpredictably moving objects presents a unique set of challenges. For example, a pre-computed robust grasp can become unreachable or unstable as the target object moves, and motion planning must also be adaptive. In this work, we present a new approach, Eye-on-hAnd Reinforcement Learner (EARL), for enabling coupled Eye-on-Hand (EoH) robotic manipulation systems to perform real-time active pose tracking and dynamic grasping of novel objects without explicit motion prediction. EARL readily addresses many thorny issues in automated hand-eye coordination, including fast-tracking of 6D object pose from vision, learning control policy for a robotic arm to track a moving object while keeping the object in the camera's field of view, and performing dynamic grasping. We demonstrate the effectiveness of our approach in extensive experiments validated on multiple commercial robotic arms in both simulations and complex real-world tasks.

==> sections/discussion.tex <==
\section{DISCUSSION AND FUTURE WORK}
\label{sec:discussion}





==> sections/intro.tex <==
\section{INTRODUCTION}
\label{sec:intro}

\begin{figure}[t!]
\vspace{2mm}
    \centering
    \includesvg[inkscapelatex=false, width = 0.98\linewidth]{figures/system.svg}
    \caption{[upper block] One of the two Eye-on-Hand (EoH) systems used in this research, in which an Intel RealSense L515 RGB-D camera is mounted over a Robotic 2-finger gripper on a Universal Robots UR-5e arm. 
    [lower block] Snapshots of EARL handling three challenging setups. (left) The EoH follows a cup and grasps it as it is placed on a tall box. (middle) The EoH tracks and grasps a box as it is moved and placed behind a ``wall''. (right) The EoH grasps a spray bottle as it is moved outside the workspace in which it is trained while also making a switch of the grasping pose. 
    \label{fig:system-snapshot}
    }
    \vspace{-5mm}
\end{figure}

Robust 6D pose tracking and grasping everyday objects constitutes a \emph{fundamental skill} for enabling the next generation of advanced robotic applications. 
%Acquiring the skill of robust 6D pose tracking and grasping of everyday objects is a crucial stepping stone toward realizing the full potential of the next generation of advanced robotic technology.
%
Despite significant recent progress in the field \cite{labbe2020cosypose, sun2022onepose, mousavian20196, wen2021catgrasp, zeng2018learning, huang2022parallel, tuscher2021deep,marturi2019dynamic, wu2022grasparl},
% Cite grasp pose generation papers, pose tracking papers, precision manipulation papers, etc. 
%
in a supermajority of vision-based manipulation systems, the perception subsystem (e.g., RGB-D cameras) and the manipulation subsystems (e.g., robot arms) are \emph{decoupled}. Typical conventional setups contain RGB-D camera(s) fixated above the workspace \cite{zeng2018learning, huang2022parallel, tuscher2021deep}, with a static camera pose often optimized for achieving the task at hand. 
% Add a figure with a typical system, and our system 
In cases where the perception system is mounted on the robot arm near the end-effector \cite{marturi2019dynamic, wu2022grasparl}, pose estimation is generally carried out afar; the perception process remains decoupled from the object manipulation operation. 
%
The independence between perception and manipulation subsystems is amenable to performing precise pose estimation and completing a \emph{pre-planned grasp}. 
%

However, these decoupled systems also have significant limitations, making them unsuitable for many practical tasks.  
%
Decoupling perception and manipulation subsystems implicitly assume ideal viewing distances to and angles of the target objects. Such assumptions require large clearance above/around the workspace surface, rendering the overall system inflexible and unsuitable for applications in confined spaces, e.g., searching for and retrieving a condiment jar in a cabinet blocked by other objects or performing inspection and repair tasks in a pipe using a snake-like robot \cite{yamada2013snake, 6225255}. 
%
Decoupling between the subsystems also requires a non-trivial time between a perception and a subsequent manipulation action. This, in turn, implies that the target objects are fully static or move with entirely predictable motions. If a target object moves unpredictably after pose estimation is performed, the ensuing grasping operation will most likely fail, making the system fragile. 
%

%Note that, as the robot end-effector moves closer to the object, 


%top right image has view  from wrist %

In this work, we introduce novel methods for enabling coupled ``Eye-on-Hand'' (EoH) robotic systems to execute \emph{active pose-tracking and grasping} tasks of unpredictably moving objects in real-time (see. Fig.~\ref{fig:system-snapshot}). A coupled EoH system effectively addresses the limitations mentioned above because it does not require perception at-a-distance and can continuously track a target object until a grasp is achieved.  
%
The binding constraint on the ``eye'' and the ``hand'' subsystems and the substantial range change for the perception system brings significant computational challenges in enabling coupled EoH systems. 
%
Nevertheless, using our approach, called \b{E}ye-on-h\b{A}nd (system) \b{R}einforcement \b{L}earner (\b{\earl}), after finding a target object and obtaining a set of initial 6D grasping poses, the EoH system approaches the object while keeping track of its pose through motion, despite drastically changing distances between the camera and the target object. 
%
\earl can be effectively trained in Isaac Gym \cite{} through a carefully designed curriculum. 
%
With \earl, an EoH system actively maintains the target object in view and within grasp until it identifies an optimum  opportunity to execute a grasping command. 
%
Through extensive evaluation, we demonstrate that \earl robustly and effectively tracks moving objects until the grasping is realized. 

%We refer to our methods as Active Pose Tracker (APT), reflecting their main function. In summary, APT makes several meaningful contributions toward the development of RGB-D vision-based prehensile manipulation capabilities for robots:
In summary, our work makes the following contributions:
\begin{itemize}[leftmargin=3.5mm]
%\vspace{-1mm}
    \item It introduces a high-performance manipulation pipeline, \earl, for achieving dynamic grasping tasks through active pose tracking, realized on general Eye-on-Hand systems consisting of an RGB-D camera mounted near the end-effector of a high-DOF robotic arm. \earl works with novel objects without an initial 3D scan. %\vspace{-4mm}
    \item It contributes a curriculum-trained reinforcement learning (RL) algorithm for deriving a control policy that can continuously track a target object with a hand-eye camera through unpredictable motion in real-time, for gradually approaching the object and executing grasping action at the optimum moment with consistently high success rates.  %\vspace{-4mm}
    \item It presents a method designed to continuously track an object in 6D ($SE(3)$) space. Therefore, our system can perform full 6D grasping for challenging tasks, including object handovers in midair. In contrast, recent approaches [9], [12], [13] mostly work with object pose changes that are confined to 3D ($SE(2)$), e.g., on a tabletop.  %\vspace{0mm}
    \item  It provides an extensive evaluation of our proposed pipeline on novel objects in extended workspaces, showing dynamic switching between grasping poses when required to complete grasping in 6D with a moving eye-on-hand camera. Coupled EoH systems powered by our methods are endowed with advanced novel capabilities, including verified native support for different robot arms (Universal Robotics UR-5e and Kinova Kortex) with virtually no sim-to-real gap after training entirely in simulation. 
    %\item We propose the first complete object-tracking and grasping algorithms for coupled EoH systems consisting of a perception system (RGB-D camera) mounted on a mechanical grasping subsystem near the end-effector. With consistently high success rates, our curriculum-trained reinforcement learning (RL) method continually tracks a target object through unpredictable motion in real-time, gradually approaches the object, and executes grasping actions when an opportunity presents itself. 
    %\item Our methods are designed to continuously track an object's pose as it moves in 6D (i.e., $SE(3)$) space. In contrast, recent approaches \cite{song2020grasping,wu2022grasparl,wang2022goal} mostly work with object pose changes that are confined to a 3D (i.e., $SE(2)$) subspace, e.g., a tabletop. As such, the resulting EoH system, powered by our methods, can successfully complete challenging tasks, including midair object handovers from a human to a robot. 
    %\item Coupled EoH systems powered by our methods are endowed with many new capabilities, including native support for multiple robot arms (Universal Robotics UR-5e and Kinova Kortex are verified)  and novel objects operating in extended workspace volumes not initially known to the perception system, and dynamic switching between multiple grasping poses when necessary. 
\end{itemize}

\begin{comment}
\textcolor{red}{JJ's edit location}
Grasping is a fundamental and challenging problem in robotics. Robotic perception, planning, and control are simultaneously required to perform grasping reliably. The problem becomes complex in unstructured scenarios, where it becomes crucial to handle the changes in the robot’s workspace, sensor noise, perception errors, inaccuracies in the robot’s control, or perturbations for performing robust and intelligent grasping. Furthermore, in real-world dynamic environments, the objects may be moving or have never been seen previously. 

In summary, our work makes the following contributions:
\begin{itemize}
  \item We use a single camera mounted on the wrist to provide RGB-D input to the system. Whereas most other works~\cite{marturi2019dynamic, akinola2021dynamic, tuscher2021deep} will use an external camera to capture the scene of the workspace and the robot.
  \item The action space of our algorithm is continuous, and the object is continuously moving in $SE(3)$ compared to~\cite{song2020grasping, wu2022grasparl, wang2022goal}. Our method can grasp an object in closed loop form for the dynamic object but also has a subgoal of keeping the object in the camera frame.
  \item We proposed two methods, one based on the Inverse kinematic of the robot (simple yet effective). The other one is the RL-based PPO algorithm which directly outputs the velocity of each joint.
  \item We integrate the object tracking, pose estimation, grasp net, RL policy for robot control as a complete pipeline to track a moving object and grasp it in real-time, which is platform-independent (no extra components needed other than a robot arm and camera on it, also tested on different robot system).
  \item Our system can also complete human-robot handover.
  \item We can switch between grasp poses if needed.
  \item Our system works on novel objects.
\end{itemize}
\end{comment}

We explore related work in Sec.~\ref{}. System setup and task description are described in Sec.~\ref{}. In Sec.~\ref{} and Sec.~\ref{}, we present the overall system pipeline and \earl, respectively. Experimental details are described in Sec.~\ref{}. We discuss future research and conclude in Sec.~\ref{}.


